A TEE-based Approach for Preserving Data Secrecy in Process Mining with Decentralized Sources

Process mining techniques enable organizations to gain insights into their business processes through the analysis of execution records (event logs) stored by information systems. While most process mining efforts focus on intra-organizational scenarios, many real-world business processes span multiple independent organizations. Inter-organizational process mining, though, faces significant challenges, particularly regarding confidentiality guarantees: The analysis of data can reveal information that the participating organizations may not consent to disclose to one another, or to a third party hosting process mining services. To overcome this issue, this paper presents CONFINE, an approach for secrecy-preserving inter-organizational process mining. CONFINE leverages Trusted Execution Environments (TEEs) to deploy trusted applications that are capable of securely mining multi-party event logs while preserving data secrecy. We propose an architecture supporting a four-stage protocol to secure data exchange and processing, allowing for protected transfer and aggregation of unaltered process data across organizational boundaries. To avoid out-of-memory errors due to the limited capacity of TEEs, our protocol employs a segmentation-based strategy, whereby event logs are transmitted to TEEs in smaller batches. We conduct a formal verification of correctness and a security analysis of the guarantees provided by the TEE core. We evaluate our implementation on real-world and synthetic data, showing that the proposed approach can handle realistic workloads. The results indicate logarithmic memory growth with respect to the event log size and linear growth with the number of provisioning organizations, highlighting scalability properties and opportunities for further optimization.

==> addon/commands-for-revisions.tex <==
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Highlight changes in revised manuscripts
%
% To color text
\RequirePackage{xcolor}
% To create side-notes
\RequirePackage{marginnote}
% To treat comma-separated input parameters (see the HlRev environment below)
\RequirePackage{xparse}
% To cross-reference the revision letter
\RequirePackage{xr}

%
%%%%%%%%%%%%%%%% Customisations
%
\def\DoShowLinksToReviewerComments{1} % Set this parameter to 1 to enable sidenotes linking a change in \HlRev (see below) to the Reviewer's comments' document. Otherwise, set it to 0.
%
% Change the following lines for larger (or narrower) side spaces
\setlength{\marginparwidth}{2.75cm}
\def\HlRevInnerWidth{2.15cm}
%
\renewcommand*{\raggedleftmarginnote}{\raggedright}
\renewcommand*{\raggedrightmarginnote}{\raggedleft}
%
% Change the following line for bigger (or smaller) fonts
\renewcommand*{\marginfont}{\normalsize}
%
%
%%%%%%%%%%%%%%%% Commands
%
\definecolor{burntorange}{rgb}{0.8, 0.33, 0.0}
\if\DoShowLinksToReviewerComments1% Add a side note with a link to the Reviewer's comment if this option is enabled (see above, under the "Customisation" section)
	\ExplSyntaxOn
	\newenvironment{HlRev}[1][]{%
		% Change the colour to orange
		\color{burntorange}%
		% If an argument is passed, it is used as the number of the comment in a side note
		\ifx\newenvironment#1\newenvironment\else%
		\marginnote{\parbox[t]{\HlRevInnerWidth}{\raggedright%
				% No hyperrefs in side-notes
				\begin{NoHyper}%
					\clist_set:Nn \l_tmpa_clist {#1}% Get the comma-separated
					\int_set:Nn \l_tmpa_int { \clist_count:N \l_tmpa_clist }
					\hspace*{0pt}% Trick to allow the first word to be hyphenised if need be
					Comment% Write ``Comment''
					\int_compare:nT { \l_tmpa_int > 1 }{s}% Add an s (Comment*s*) if there are multiple comments inside
					{\ #1}% Write the referred comment(s)
					% Restores the normal hyperref behaviour
				\end{NoHyper}%
		}}%
		\fi%
		%
	}{%
		% Restores the normal colour
		\normalcolor%
	}%
	\ExplSyntaxOff%
\else%
	\newenvironment{HlRev}[1][]{%
	% Change the colour to orange
	\color{burntorange}
	}{%
	% Restores the normal colour
	\normalcolor%
	}%
\fi

% Defines the path for the main accompanying letter file (so as to cross-reference reviewers' remarks by prepending "letter:" to the original label )
\externaldocument[letter:]{../src-letter/letter}

%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%


==> algorithms/confine.tex <==
% !TeX encoding = utf8
% !TeX root = ../main.tex
%
\begin{comment}
	% See macros file
	\def\LPrv {\ensuremath{\mathcal{P}}}   % Log provider
	\def\SecM {\ensuremath{\mathcal{M}}}   % Secure Miner
	\def\LPrvS {\ensuremath{\widehat{\mathcal{P}}}}  % Log provider set
	\def\CStor {\ensuremath{\textrm{Cases}}}  % Case store 
	\def\Case {\ensuremath{c}}  % Case 
	\def\CasP {\ensuremath{\textrm{casePart}}}  % Case part
	\def\CId {\ensuremath{\textrm{cid}}}  % CaseId
	\def\CIdU {\ensuremath{\widehat{\textrm{CID}}}}  % CaseId universe
	\def\CS {\ensuremath{C}}  % Case set
	\def\CasU {\ensuremath{\widehat{C}}}  % Case universe
	\def\CIdS {\ensuremath{\textrm{CIDs}}}  % CaseId set
	\def\CIDMap {\ensuremath{\textrm{CIDMap}}} % CaseId Map
	\def\LPrvMap {\ensuremath{\textrm{PMap}}} % Log provider Map
	\newcommand{\Mesg}[1]{\ensuremath{\textrm{\textsc{#1}}}}
	\newcommand{\SuchThat}[1]{~\upshape\textrm{\textbf{such that}}~{#1}}
	\newcommand{\To}[1]{~\upshape\textrm{\textbf{to}}~{#1}}
	\newcommand{\Call}[1]{\texttt{#1}}
	
	\def\SegSize {\ensuremath{\textrm{seg\_size}}}
	\def\Segm {\ensuremath{S}}
\end{comment}

\tiny
% \scriptsize
\DontPrintSemicolon \SetAlgoVlined
\SetKw{Trigger}{trigger}
\SetKw{Yield}{yield}
\SetKw{Return}{return}
\SetKwProg{UponEv}{upon event}{ do}{}
\SetKwProg{Upon}{upon}{ do}{}
\SetKwInput{Implements}{Implements}
\SetKwInput{Uses}{Uses}
\SetKwProg{Fn}{Function}{ is}{}
\def\self {\ensuremath{\textrm{self}}}

\KwIn{%
	$\LPrvS = \{ \LPrv_1, \ldots, \LPrv_n \}$, the (references to) $n$ log provisioners;%
	\newline
	$\SegSize$, the maximum size of the log segment to be transmitted by the log provisioners;%
	%	\newline%
	%	$\DecRepertoire$, a finite set of {\Declare} templates to be considered to express the discovered specification;%
	%	\newline%
	%	$\ProActvts \subseteq \Uact$, a finite set of activities to be included in the discovered specification;%
	%	\newline%
	%	$\MinThrld{\ConfTr}$, $\MinThrld{\SuppTr}$, $\MinThrld{\ConfEv}$, $\MinThrld{\SuppEv}$, the minimum thresholds for trace-based confidence and support, and event-based confidence and support, respectively (default for all four paramenters: $0.0$); %the minimum support 
}
\KwData{%
	$\CIDMap : \CIdU \to 2^{\LPrvS}$, a map from case references $\CId \in \CIdU$ to the set of log provisioners in $\LPrvS$ ; \newline%
	$\LPrvMap : \LPrvS \to 2^{\CIdU}$, a map from log provisioners $\LPrv \in \LPrvS$ to the set of references to their cases in $\CIdU$ ; \newline%
	$\CStor : \CIdU \to \CasU$, a map from case references $\CId \in \CIdU$ to a set of cases in $\CasU$
}
%\KwOut{%
	%	$\DecSpec$, a declarative process specification
	%}
\Implements{\Compo{SecureMiner} \SecM}
\Uses{\Compo{LogProvisioner} \LPrv}

\begin{comment}
	\todo{For an extended version, we should enlarge this pseudocode with the full interface}
	\Fn{\Call{getAttestationReport}(\LPrv) \SuchThat{$\LPrv \in \LPrvS$} \label{alg:getAttestationReport}}{
		\Return {attestation\_report}
	}
\end{comment}

\BlankLine
% 
%\ForEach{$\LPrv \in \LPrvS$ \tcc*[r]{For every log provider $\LPrv$}}{%
	%	$\CaseIdS \gets \CaseIdS \cup \LPrv.\CaseIdS$; \tcc*[r]{Register the $\LPrv$'s case reference list}%
	%	
	%}
\UponEv(\tcp*[f]{The \textit{initialization} phase begins here -- \cref{fig:init}}){\upshape $\langle \SecM.\Compo{LogRequester}, \Mesg{Init} \:|\: \LPrvS, \SegSize \rangle$}{
	\ForEach(\tcp*[f]{Request the list of cases provided by every \Compo{Log Provider} $\LPrv$}){$\LPrv \in \LPrvS$}{%
		\Trigger{\upshape $\langle \LPrv.\Compo{LogProvider}, \Mesg{CaseRefsReq} \rangle$\label{alg:CaseRefsReq:call}} \tcp*{$\LPrv$ will reply with \Mesg{CaseRefsRes} (see line~\ref{alg:CaseRefsRes})}
	}
	\Upon(\tcp*[f]{Once all $\LPrv$s have answered, the \Compo{Secure Miner} requests their cases}){\upshape $|\LPrvS| = |\textrm{dom}(\LPrvMap)|$}{%
		\lForEach%(\tcp*[f]{For every reference to the \Compo{Log Provider} $\LPrv'$})
		{$\LPrv \in \LPrvS$}{
			\Trigger{\upshape $\langle \LPrv.\Compo{LogProvider}, \Mesg{CasesReq} \:|\: \LPrv, \SegSize, \LPrvMap[\LPrv] \rangle$\label{alg:CasesReq:call}}
			\tcp*[f]{(see line~\ref{alg:CasesReq})}
			%\tcc*{Request the cases that are provided by $\LPrv'$. Before sending them, $\LPrv'$ will trigger \Mesg{AttestReportReq} in return, to attest the \Compo{Secure Miner}.}
		}
	}
}
\UponEv(\tcp*[f]{{\SecM} gets case references (line~\ref{alg:CaseRefsReq:call})}){\upshape $\langle \SecM.\Compo{LogRequester}, \Mesg{CaseRefsRes} \:|\: \LPrv, \CIdS \rangle$ \SuchThat{$\LPrv \in \LPrvS$} \label{alg:CaseRefsRes}}{
	\ForEach(\tcp*[f]{For every reference to a case $\CId$}){\upshape $\CId \in \CIdS$}{%
		$\CIDMap[\CId] \gets \CIDMap[\CId] \cup \{\LPrv\} $ \tcp*{Add $\LPrv$ to the set of providers for case $\CId$ in $\CIDMap$}
	}
	$\LPrvMap[\LPrv] \gets \LPrvMap[\LPrv] \cup \CIdS $ \tcp*{Register the references of the cases provided by $\LPrv$ in $\LPrvMap$}
}
\UponEv(\tcp*[f]{The \Compo{Log Provider} gets the case request (line~\ref{alg:CasesReq:call})}){\upshape$\langle \LPrv.\Compo{LogProvider}, \Mesg{CasesReq} \:|\: \SecM, \SegSize, \CIdS \rangle$ \label{alg:CasesReq}}{%
	\If(\tcp*[f]{The \textit{attestation phase} (see \cref{fig:attestation})}){\upshape \SecM.\Compo{LogReceiver}.\Call{getAttestationReport}(\LPrv) is valid}{
		$\{\Segm_1, \ldots, \Segm_m\} \gets \LPrv.\Compo{LogProvider}.\Call{segmentEventLog}( \Compo{LogRecorder}.\Call{accessEventLog}(\CIdS), \SegSize )$ \tcp*[f]{Split by \SegSize} \\
		\ForEach(\tcp*[f]{For every split segment}){$i \in \{1, \ldots, m\}$}{%
			\Trigger{\upshape $\langle \SecM.\Compo{LogReceiver}, \Mesg{CasesRes} \:|\: \LPrv, \Segm_i \rangle$ } \tcp*[f]{\LPrv sends segments to {\SecM} (see line \ref{alg:CasesRes})} \label{alg:sendSegs}
		}
	}
}
\UponEv(\tcp*[f]{$\SecM$ gets segments (line \ref{alg:sendSegs})}){\upshape $\langle \SecM.\Compo{LogReceiver}, \Mesg{CasesRes} \:|\: \LPrv, \Segm \rangle$ \SuchThat{$\LPrv \in \LPrvS$} \label{alg:CasesRes} }{
	% See {\LaTeX} comments\\
	% Per ogni pezzo-di-caso ricevuto nel segmento, controlla che il provider sia stato dichiarato in possesso di esso
	% SE PMap ha ancora il CID
	% Aggiungi il pezzo-di-caso alla lista di pezzi-di-caso associati a quell'id
	% Togli il CID del pezzo-di-caso da PMap in P
	% Togli il P dal CIDMap
	% upon CIDMap vuoto in un CID, mergia e yielda il caso
	\ForEach(\tcp*[f]{For every $\CasP_\CId$ in the delivered set of segments $\Segm$, each associated with a \CId}){\upshape $\CasP_\CId \in \Segm$}{%
		\If(\tcp*[f]{The store phase (see \cref{fig:transmission})}){\upshape $\CId \in \LPrvMap[\LPrv]$}  {%
			$\LPrvMap[\LPrv] \gets \LPrvMap[\LPrv] \,\setminus\, \{\CId\}$ \tcp*[f]{\raggedright Remove {\CId} from the set of cases to be provided by {\LPrv}}\;
			$\CIDMap[\CId] \gets \CIDMap[\CId] \,\setminus\, \{\LPrv\}$ \tcp*[f]{Remove $\LPrv$ from the set of $\CId$ providers}\;
			$\Compo{LogManager}.\Call{mergeAndStore}\left(\CStor, \CasP_\CId\right)$ \tcp*[f]{Update the case via $\Merge$ and store the result in {\CStor}}
		}
	}
}

\Upon(\tcp*[f]{When all the pieces of some $\CId$ have arrived}){\upshape $\CIDMap[\CId]= \emptyset$ for some $\CId \in \textrm{dom}(\CIDMap)$} {%
	$\textrm{dom}(\CIDMap) \gets \textrm{dom}(\CIDMap) \,\setminus\, \{\CId\}$\tcp*[f]{Remove $\CId$ from the $\CId$ domain which still needs to be processed}\;
	\Yield{\upshape \CStor[\CId] \To{}} \Compo{LogProcessor} \tcp*[f]{\Compo{Log Manager} forwards the $\CId$ to the \Compo{Log Processor} for mining (\cref{fig:computation})}
}

\endinput
UPON EVENT(M,CASERES|P,S) SUCH THAT P in \widehat{\mathcal{P}} DO
	for each C ∈ S:
		if C.cid ∈ PMap[P]
			CMap[C.cid]<--CMap[C.cid] ∪ {C}
			PMap[P]<-- PMap[P] \ {C.cid}
			CIDMap[C.cid]<-- CIDMap[C.cid] \ {P}


UPON |CIDMap[cid]|=0 such that cid in dom(CIDMap) //Computation phase start here.
merge all traces in CIDMap[cid] using mergingSchema and put it in mergedTrace
yeld PMAlgorithm(mergedTrace)


==> algorithms/confineBackup.tex <==
% !TeX encoding = utf8
% !TeX root = ../main.tex
%
\begin{comment}
	% See macros file
	\def\LPrv {\ensuremath{\mathcal{P}}}   % Log provider
	\def\SecM {\ensuremath{\mathcal{M}}}   % Secure Miner
	\def\LPrvS {\ensuremath{\widehat{\mathcal{P}}}}  % Log provider set
	\def\CStor {\ensuremath{\textrm{Cases}}}  % Case store 
	\def\Case {\ensuremath{c}}  % Case 
	\def\CasP {\ensuremath{\textrm{casePart}}}  % Case part
	\def\CId {\ensuremath{\textrm{cid}}}  % CaseId
	\def\CIdU {\ensuremath{\widehat{\textrm{CID}}}}  % CaseId universe
	\def\CS {\ensuremath{C}}  % Case set
	\def\CasU {\ensuremath{\widehat{C}}}  % Case universe
	\def\CIdS {\ensuremath{\textrm{CIDs}}}  % CaseId set
	\def\CIDMap {\ensuremath{\textrm{CIDMap}}} % CaseId Map
	\def\LPrvMap {\ensuremath{\textrm{PMap}}} % Log provider Map
	\newcommand{\Mesg}[1]{\ensuremath{\textrm{\textsc{#1}}}}
	\newcommand{\SuchThat}[1]{~\upshape\textrm{\textbf{such that}}~{#1}}
	\newcommand{\To}[1]{~\upshape\textrm{\textbf{to}}~{#1}}
	\newcommand{\Call}[1]{\texttt{#1}}
	
	\def\SegSize {\ensuremath{\textrm{seg\_size}}}
	\def\Segm {\ensuremath{S}}
\end{comment}

\tiny
% \scriptsize
\DontPrintSemicolon \SetAlgoVlined
\SetKw{Trigger}{trigger}
\SetKw{Yield}{yield}
\SetKw{Return}{return}
\SetKwProg{UponEv}{upon event}{ do}{}
\SetKwProg{Upon}{upon}{ do}{}
\SetKwInput{Implements}{Implements}
\SetKwInput{Uses}{Uses}
\SetKwProg{Fn}{Function}{ is}{}
\def\self {\ensuremath{\textrm{self}}}

\KwIn{%
	$\LPrvS \ni \{ \LPrv_1, \ldots, \LPrv_n \}$, the (references to) $n$ log provisioners;%
	\newline
	$\SegSize$, the maximum size of the log segment to be transmitted by the log provisioners;%
	%	\newline%
	%	$\DecRepertoire$, a finite set of {\Declare} templates to be considered to express the discovered specification;%
	%	\newline%
	%	$\ProActvts \subseteq \Uact$, a finite set of activities to be included in the discovered specification;%
	%	\newline%
	%	$\MinThrld{\ConfTr}$, $\MinThrld{\SuppTr}$, $\MinThrld{\ConfEv}$, $\MinThrld{\SuppEv}$, the minimum thresholds for trace-based confidence and support, and event-based confidence and support, respectively (default for all four paramenters: $0.0$); %the minimum support 
}
\KwData{%
	$\CIDMap : \CIdU \to 2^{\LPrvS}$, a map from case references $\CId \in \CIdU$ to the set of log provisioners in $\LPrvS$ ; \newline%
	$\LPrvMap : \LPrvS \to 2^{\CIdU}$, a map from log provisioners $\LPrv \in \LPrvS$ to the set of references to their cases in $\CIdU$ ; \newline%
	$\CStor : \CIdU \to \CasU$, a map from case references $\CId \in \CIdU$ to a set of case parts in $\CasU$
}
%\KwOut{%
	%	$\DecSpec$, a declarative process specification
	%}
\Implements{\Compo{SecureMiner} \SecM}
\Uses{\Compo{LogProvisioner} \LPrv}

\begin{comment}
	\todo{For an extended version, we should enlarge this pseudocode with the full interface}
	\Fn{\Call{getAttestationReport}(\LPrv) \SuchThat{$\LPrv \in \LPrvS$} \label{alg:getAttestationReport}}{
		\Return {attestation\_report}
	}
\end{comment}

\BlankLine
% 
%\ForEach{$\LPrv \in \LPrvS$ \tcc*[r]{For every log provider $\LPrv$}}{%
	%	$\CaseIdS \gets \CaseIdS \cup \LPrv.\CaseIdS$; \tcc*[r]{Register the $\LPrv$'s case reference list}%
	%	
	%}
\UponEv(\tcp*[f]{The \textit{initialization} phase begins here -- \cref{fig:init}}){\upshape $\langle \SecM.\Compo{LogRequester}, \Mesg{Init} \:|\: \LPrvS, \SegSize \rangle$}{
	\ForEach(\tcp*[f]{Request the list of cases provided by every \Compo{Log Provider} $\LPrv$}){$\LPrv \in \LPrvS$}{%
		\Trigger{\upshape $\langle \LPrv.\Compo{LogProvider}, \Mesg{CaseRefsReq} \rangle$\label{alg:CaseRefsReq:call}} \tcp*{$\LPrv$ will reply with \Mesg{CaseRefsRes} (see line~\ref{alg:CaseRefsRes})}
	}
	\Upon(\tcp*[f]{Once all $\LPrv$s have answered, the \Compo{Secure Miner} requests their cases}){\upshape $|\LPrvS| = |\textrm{dom}(\LPrvMap)|$}{%
		\lForEach%(\tcp*[f]{For every reference to the \Compo{Log Provider} $\LPrv'$})
		{$\LPrv \in \LPrvS$}{
			\Trigger{\upshape $\langle \LPrv.\Compo{LogProvider}, \Mesg{CasesReq} \:|\: \LPrv, \SegSize, \LPrvMap[\LPrv] \rangle$\label{alg:CasesReq:call}}
			\tcp*[f]{(see line~\ref{alg:CasesReq})}
			%\tcc*{Request the cases that are provided by $\LPrv'$. Before sending them, $\LPrv'$ will trigger \Mesg{AttestReportReq} in return, to attest the \Compo{Secure Miner}.}
		}
	}
}
\UponEv(\tcp*[f]{{\SecM} gets case references (line~\ref{alg:CaseRefsReq:call})}){\upshape $\langle \SecM.\Compo{LogRequester}, \Mesg{CaseRefsRes} \:|\: \LPrv, \CIdS \rangle$ \SuchThat{$\LPrv \in \LPrvS$} \label{alg:CaseRefsRes}}{
	\ForEach(\tcp*[f]{For every reference to a case $\CId$}){$\CId \in \CIdS$}{%
		$\CIDMap[\CId] \gets \CIDMap[\CId] \cup \{\LPrv\} $ \tcp*{Add $\LPrv$ to the set of providers for case $\CId$ in $\CIDMap$}
	}
	$\LPrvMap[\LPrv] \gets \LPrvMap[\LPrv] \cup \CIdS $ \tcp*{Register the references of the cases provided by $\LPrv$ in $\LPrvMap$}
}
\UponEv(\tcp*[f]{The \Compo{Log Provider} gets the case request (line~\ref{alg:CasesReq:call})}){\upshape$\langle \LPrv.\Compo{LogProvider}, \Mesg{CasesReq} \:|\: \SecM, \SegSize, \CIdS \rangle$ \label{alg:CasesReq}}{%
	\If(\tcp*[f]{The \textit{attestation phase} (see \cref{fig:attestation})}){\upshape \SecM.\Compo{LogReceiver}.\Call{getAttestationReport}(\LPrv) is valid}{
		$\{\Segm_1, \ldots, \Segm_m\} \gets \Call{segmentEventLog}( \Compo{LogRecorder}.\Call{accessEventLog}(\CIdS), \SegSize )$\\
		\ForEach{$i \in \{1, \ldots, m\}$}{%
			\Trigger{\upshape $\langle \SecM.\Compo{LogReceiver}, \Mesg{CasesRes} \:|\: \LPrv, \Segm_i \rangle$ }
		}
	}
}
\UponEv{\upshape $\langle \SecM.\Compo{LogReceiver}, \Mesg{CasesRes} \:|\: \LPrv, \Segm \rangle$ \SuchThat{$\LPrv \in \LPrvS$}}{
	% See {\LaTeX} comments\\
	% Per ogni pezzo-di-caso ricevuto nel segmento, controlla che il provider sia stato dichiarato in possesso di esso
	% SE PMap ha ancora il CID
	% Aggiungi il pezzo-di-caso alla lista di pezzi-di-caso associati a quell'id
	% Togli il CID del pezzo-di-caso da PMap in P
	% Togli il P dal CIDMap
	% upon CIDMap vuoto in un CID, mergia e yielda il caso
	\ForEach{\upshape $\CasP \in \Segm$}{%
		\If{\upshape $\Call{\CId}(\CasP) \in \LPrvMap[\LPrv]$}{%
			$\LPrvMap[\LPrv] \gets \LPrvMap[\LPrv] \,\setminus\, \{\Call{\CId}(\CasP)\}$ \;
			$\CIDMap[\Call{\CId}(\CasP)] \gets \CIDMap[\Call{\CId}(\CasP)] \,\setminus\, \{\LPrv\}$ \;
			$\Compo{LogManager}.\Call{mergeAndStore}(\CStor, {\CId}(\CasP), \CasP)$
		}
	}
}

\Upon{\upshape $\CIDMap[\CId]= \emptyset$ for some $\CId \in \textrm{dom}(\CIDMap)$} {%
	$\textrm{dom}(\CIDMap) \gets \textrm{dom}(\CIDMap) \,\setminus\, \{\CId\}$ \;
	\Yield{\upshape \CStor[\CId] \To{}} \Compo{LogProcessor}
}

\endinput
UPON EVENT(M,CASERES|P,S) SUCH THAT P in \widehat{\mathcal{P}} DO
	for each C ∈ S:
		if C.cid ∈ PMap[P]
			CMap[C.cid]<--CMap[C.cid] ∪ {C}
			PMap[P]<-- PMap[P] \ {C.cid}
			CIDMap[C.cid]<-- CIDMap[C.cid] \ {P}


UPON |CIDMap[cid]|=0 such that cid in dom(CIDMap) //Computation phase start here.
merge all traces in CIDMap[cid] using mergingSchema and put it in mergedTrace
yeld PMAlgorithm(mergedTrace)


==> algorithms/provisioningConf.tex <==
\tiny
% \scriptsize
\DontPrintSemicolon \SetAlgoVlined \SetInd{0.3em}{1em}
\setstretch{1.1}
% Additional macros in addon/macros.tex and addon/utils.tex

\KwIn{%
	$\SecMS = \{ \SecM_1, \ldots, \SecM_s \}$, the (references to) $s$ miners.%
}

\Implements{\Compo{Provisioner}, {\Inst} {\LPrv}.}
\Uses{\textit{AuthenticatedPerfectPointToPointLink}, {\Inst} {\AuthPtP}.}
\UponEv(\tcp*[f]{{\LPrv} receives the request for case references from {\SecM} (see \crefalgln[alg:secm]{alg:secm:CaseRefsReq:call})}){$\langle \AuthPtP, \Mesg{Deliver} \ll \SecM \:|\: \Mesg{CasesRefsReq} \rangle$ \label{alg:lprv:CasesRefReq}\SuchThat{$\SecM \in \SecMS$}}{%
	%\If(\tcp*[f]{Authenticate the sender miner {\SecM}}){\LPrv.\Compo{LogProvider}.\Call{authenticateMiner}(\SecM) is successful}{
            $\CIdS \gets \LPrv.{\Compo{LogRecorder}}.\Call{accessCaseReferences()}$\tcp*[f]{Access the case references via \Compo{Log Recorder}}\\
            \Trigger{$\langle \AuthPtP, \Mesg{Send} \gg \SecM \:|\: \Mesg{CasesRefRes},\CIdS \rangle$ } \tcp*[f]{{send the case references to {\SecM} (see \crefalgln[alg:secm]{alg:secm:CaseRefsRes})\label{alg:lprv:sendRefs}}}
	%}
}
\UponEv(\tcp*[f]{{\LPrv} gets the case request from {\SecM} (see \crefalgln[alg:secm]{alg:secm:CasesReq:call})}){$\langle \AuthPtP, \Mesg{Deliver} \ll \SecM \:|\: \Mesg{CasesReq},\SegSize, \CIdS\rangle$ \label{alg:lprv:CasesReq}\SuchThat{$\SecM \in \SecMS$}}{%
	\If(\tcp*[f]{Get and verify the attestation report of {\SecM} -- \textit{remote attestation} in \cref{fig:attestation}}){\SecM.\Compo{LogReceiver}.\Call{getAttestationReport}(\LPrv) is valid \label{alg:lprv:attestation}}{
		$\{\Segm_1, \ldots, \Segm_m\} \gets \LPrv.\Compo{LogProvider}.\Call{segmentEventLog}(\LPrv.\Compo{LogRecorder}.\Call{accessEventLog}(\CIdS), \SegSize \label{alg:lprv:logaccess})$\tcp*[f]{Segment the event log} \\
		\ForEach(\tcp*[f]{For every split segment $\Segm_i$}){$i \in \{1, \ldots, m\}$}{%
			\Trigger{$\langle \AuthPtP, \Mesg{Send} \gg \SecM \:|\: \Mesg{CasesRes},\Segm_i \rangle$ } \tcp*[f]{send the segment $\Segm_i$ to {\SecM} (see \crefalgln[alg:secm]{alg:secm:CasesRes}) -- \textit{data transmission} phase in \cref{fig:transmission}} \label{alg:lprv:sendSegs}
		}
	}
}

==> algorithms/secure-miner-activity.tex <==
% !TeX encoding = utf8
% !TeX root = ../main.tex
%
\def\LPrv {\ensuremath{\mathcal{P}}}   % Log provider
\def\SecM {\ensuremath{\mathcal{M}}}   % Secure Miner
\def\LPrvS {\ensuremath{\widehat{\mathcal{P}}}}  % Log provider set
\def\Case {\ensuremath{c}}  % Case 
\def\CId {\ensuremath{\textrm{cid}}}  % CaseId
\def\CIdU {\ensuremath{\widehat{\textrm{CID}}}}  % CaseId universe
\def\CS {\ensuremath{C}}  % Case set
\def\CIdS {\ensuremath{\textrm{CIDs}}}  % CaseId set
\def\CIDMap {\ensuremath{\textrm{CIDMap}}} % CaseId Map
\def\LPrvMap {\ensuremath{\textrm{PMap}}} % Log provider Map
\newcommand{\Mesg}[1]{\ensuremath{\textrm{\textsc{#1}}}}
\newcommand{\SuchThat}[1]{~\upshape\textrm{\textbf{such that}}~{#1}}
\newcommand{\Call}[1]{\textrm{#1}}

\def\SegSize {\ensuremath{\textrm{seg\_size}}}
\def\Segm {\ensuremath{S}}

\tiny
% \scriptsize
\DontPrintSemicolon \SetAlgoVlined
\SetKw{Trigger}{trigger}
\SetKw{Return}{return}
\SetKwProg{UponEv}{upon event}{ do}{}
\SetKwProg{Upon}{upon}{ do}{}
\SetKwInput{Implements}{Implements}
\SetKwInput{Uses}{Uses}
\SetKwProg{Fn}{Function}{ is}{}
\def\self {\ensuremath{\textrm{self}}}

\KwIn{%
	$\LPrvS \ni \{ \LPrv_1, \ldots, \LPrv_n \}$, the (references to) $n$ \Compo{Log Provider}s;%
	\newline
	$\SegSize$, the maximum size of the log segment to be transmitted by the \Compo{Log Provider}s;%
%	\newline%
%	$\DecRepertoire$, a finite set of {\Declare} templates to be considered to express the discovered specification;%
%	\newline%
%	$\ProActvts \subseteq \Uact$, a finite set of activities to be included in the discovered specification;%
%	\newline%
%	$\MinThrld{\ConfTr}$, $\MinThrld{\SuppTr}$, $\MinThrld{\ConfEv}$, $\MinThrld{\SuppEv}$, the minimum thresholds for trace-based confidence and support, and event-based confidence and support, respectively (default for all four paramenters: $0.0$); %the minimum support 
}
\KwData{%
	$\CIDMap : \CIdU \to 2^{\LPrvS}$, a map from case references $\CId \in \CIdU$ to the set of log providers $\LPrv \in \LPrvS$ \newline%
	$\LPrvMap : \LPrvS \to 2^{\CIdU}$, a map from log providers $\LPrv \in \LPrvS$ to the set of references to their cases $\CId \in \CIdU$
}
%\KwOut{%
%	$\DecSpec$, a declarative process specification
%}
\Implements{\Compo{Secure Miner} \SecM}
\Uses{\Compo{Log Provider} \LPrv}

\Fn{\Call{getAttestationReport}(\LPrv) \SuchThat{$\LPrv \in \LPrvS$} \label{alg:getAttestationReport}}{
	\Return {attestation\_report}
}

\BlankLine
% 
%\ForEach{$\LPrv \in \LPrvS$ \tcc*[r]{For every log provider $\LPrv$}}{%
%	$\CaseIdS \gets \CaseIdS \cup \LPrv.\CaseIdS$; \tcc*[r]{Register the $\LPrv$'s case reference list}%
%	
%}
\UponEv(\tcp*[f]{The \textit{initialization} phase begins here -- \cref{fig:init}}){$\langle \SecM, \Mesg{Init} \:|\: \LPrvS, \SegSize \rangle$}{
	\ForEach(\tcp*[f]{Request the list of cases provided by every \Compo{Log Provider} $\LPrv$}){$\LPrv \in \LPrvS$}{%
		\Trigger{$\langle \LPrv, \Mesg{CaseRefsReq} \rangle$\label{alg:CaseRefsReq:call}} \tcp*{$\LPrv$ will reply with \Mesg{CaseRefsRes} (see line~\ref{alg:CaseRefsRes})}
	}
	\Upon(\tcp*[f]{Once all $\LPrv$s have answered, the \Compo{Secure Miner} requests their cases\ldots}){\upshape $|\LPrvS| = |\textrm{dom}(\LPrvMap)|$}{%
	\lForEach%(\tcp*[f]{For every reference to the \Compo{Log Provider} $\LPrv'$})
		{$\LPrv \in \LPrvS$}{
			\Trigger{\upshape $\langle \LPrv, \Mesg{CasesReq} \:|\: \self, \SegSize \rangle$\label{alg:CasesReq:call}}
			\tcp*[f]{\ldots specifying the {\SegSize} (see line~\ref{alg:CasesReq})}
			%\tcc*{Request the cases that are provided by $\LPrv'$. Before sending them, $\LPrv'$ will trigger \Mesg{AttestReportReq} in return, to attest the \Compo{Secure Miner}.}
		}
	}
}
\UponEv(\tcp*[f]{{\SecM} receives {\LPrv}'s case references (line~\ref{alg:CaseRefsReq:call})}){$\langle \SecM, \Mesg{CaseRefsRes} \:|\: \LPrv, \CIdS \rangle$ \SuchThat{$\LPrv \in \LPrvS$} \label{alg:CaseRefsRes}}{
	\ForEach(\tcp*[f]{For every reference to a case $\CId$}){$\CId \in \CIdS$}{%
		$\CIDMap[\CId] \gets \CIDMap[\CId] \cup \{\LPrv\} $ \tcp*{Add $\LPrv$ to the set of providers for case $\CId$ in $\CIDMap$}
	}
	$\LPrvMap[\LPrv] \gets \LPrvMap[\LPrv] \cup \CIdS $ \tcp*{Register the references of the cases provided by $\LPrv$ in $\LPrvMap$}
}
\UponEv(\tcp*[f]{The \Compo{Log Provider} receives the request for cases (see line~\ref{alg:CasesReq:call})}){$\langle \LPrv, \Mesg{CasesReq} \:|\: \SecM, \SegSize \rangle$ \label{alg:CasesReq}}{%
	\If(\tcp*[f]{The \textit{attestation phase} (see \cref{fig:attestation} and line~\ref{alg:getAttestationReport})}){\SecM.\Call{getAttestationReport}(\LPrv) is valid}{
		$\{\Segm_1, \ldots, \Segm_m\} \gets \Call{segmentEventLog}( \Call{accessEventLog}(), \SegSize )$ \\
		\ForEach{$\Segm \in \{\Segm_1, \ldots, \Segm_m\}$}{%
			\Trigger{$\langle \SecM, \Mesg{CasesRes} \:|\: \self, \Segm \rangle$ }
		}
	}
}
\UponEv{$\langle \SecM, \Mesg{CasesRes} \:|\: \LPrv, \Segm \rangle$ \SuchThat{$\LPrv \in \LPrvS$}}{
	See {\LaTeX} comments\\
	% Per ogni pezzo-di-caso ricevuto nel segmento, controlla che il provider sia stato dichiarato in possesso di esso
	% SE PMap ha ancora il CID
		% Aggiungi il pezzo-di-caso alla lista di pezzi-di-caso associati a quell'id
		% Togli il CID del pezzo-di-caso da PMap in P
		% Togli il P dal CIDMap
	% upon CIDMap vuoto in un CID, mergia e yielda il caso
        
}       

\endinput

\KwOut{%
	$\DecSpec$, a declarative process specification
}
%
\BlankLine
$ \CnsSet \gets \left\{ \DecTemp(a_1, \ldots, a_m) : \DecTemp \in \DecRepertoire, a_1; \ldots, a_m \in \ProActvts, a_i \neq a_j \textrm{ with } 1 \leq i,j \leq m \right\}$\; \tcc*[r]{candidate constraints: templates assigned with any pair of distinct activities} \label{alg:candidates}
\BlankLine
%
\ForEach{$ \Cns \in\CnsSet $ \tcc*[r]{compute measures} }{
	$\mathrm{c_\textrm{t}} \gets \ConfTrOf{\Cns}{\EvtLog}$;
	$\mathrm{s_\textrm{e}} \gets \SuppTrOf{\Cns}{\EvtLog}$;
	$\mathrm{c_\textrm{e}} \gets \ConfEvOf{\Cns}{\EvtLog}$;
	$\mathrm{s_\textrm{e}} \gets \SuppEvOf{\Cns}{\EvtLog}$\;
	\If{${ c_\textrm{t} \leq \MinThrld{\ConfTr} } \textrm{ or }
		{ s_\textrm{t} \leq \MinThrld{\SuppTr} } \textrm{ or }
		{ c_\textrm{e} \leq \MinThrld{\ConfEv} } \textrm{ or }
		{ s_\textrm{e} \leq \MinThrld{\SuppEv} }$
	}{$ \CnsSet \gets \CnsSet \setminus \{ \Cns \}$ \tcc*[r]{remove constraints with a measure below the threshold}}
} 
%
% \BlankLine
%
\ForEach{$ \Cns \in \CnsSet $ \tcc*[r]{remove constraints as per subsumption hierarchy and negated v.} }{
	\ForEach{${ \Cns' \in \CnsSet }$ s.t.\ ${ \Cns' \sqsubseteq \Cns }$ \tcc*[r]{for every $\Cns'$ that subsumes $\Cns$ in $\CnsSet$}}{
		\uIf{$\AllMsrsOf{\Cns'}{\EvtLog} \leq \AllMsrsOf{\Cns}{\EvtLog}$ \tcc*[r]{if the measures of $\Cns'$ are $\leq$ those of $\Cns$}}
		%		\If{${ \ConfTrOf{\Cns'}{\EvtLog} \geq \ConfTrOf{\Cns'}{\EvtLog} } \textrm{ and }
			%			 { \SuppTrOf{\Cns}{\EvtLog} \leq \SuppTrOf{\Cns}{\EvtLog} } \textrm{ and }
			%			 { \ConfEvOf{\Cns}{\EvtLog} \leq \ConfEvOf{\Cns}{\EvtLog} } \textrm{ and }
			%			 { \SuppEvOf{\Cns}{\EvtLog} \leq \SuppEvOf{\Cns}{\EvtLog} }$
			{ $ \CnsSet \gets \CnsSet \setminus \{ \Cns \}$ }
			\lElse{ $ \CnsSet \gets \CnsSet \setminus \{ \Cns' \}$ }%
		}
		\ForEach{${ \Cns' \in \DecSpec }$ s.t.\ $\Cns'$ is the negated version of $\Cns$ }{
			\lIf{$\AllMsrsOf{\Cns'}{\EvtLog} < 
				\AllMsrsOf{\Cns}{\EvtLog}$ }
			{ $ \CnsSet \gets \CnsSet \setminus \{ \Cns \}$ }
			\lElse{ $ \CnsSet \gets \CnsSet \setminus \{ \Cns' \}$ }%
		}
	} 
	\BlankLine
	\Return $\DecSpec = \left( \DecRepertoire, \ProActvts, \CnsSet \right)$\;

==> algorithms/secureMinerConf.tex <==
% !TeX encoding = utf8
% !TeX root = ../main.tex
%
\tiny
% \scriptsize
\DontPrintSemicolon \SetAlgoVlined \SetInd{0.3em}{1em}
\setstretch{1.1}
% Additional macros in addon/macros.tex and addon/utils.tex

\KwIn{%
	$\LPrvS = \{ \LPrv_1, \ldots, \LPrv_n \}$, the (references to) $n$ log provisioners;%
	\newline
	$\SegSize$, the maximum size of the log segment to be transmitted by the log provisioners.%
}
\KwData{%
	$\CIDMap : \CIdU \to 2^{\LPrvS}$, a map from case references $\CId \in \CIdU$ to the set of log provisioners in $\LPrvS$ ; \newline%
	$\LPrvMap : \LPrvS \to 2^{\CIdU}$, a map from log provisioners $\LPrv \in \LPrvS$ to the set of references to their cases in $\CIdU$ ; \newline%
	$\CStor : \CIdU \to \CasU$, a map from case references $\CId \in \CIdU$ to a set of cases in $\CasU$.
}
%\KwOut{%
	%	$\DecSpec$, a declarative process specification
	%}
\Implements{\Compo{SecureMiner}, {\Inst} {\SecM.}}
%\Uses{\Compo{Provisioner} \LPrv}
\Uses{\textit{AuthenticatedPerfectPointToPointLink}, {\Inst} {\AuthPtP.}}

\begin{comment}
    \todo{For an extended version, we should enlarge this pseudocode with the full interface}
    \Fn{\Call{getAttestationReport}(\LPrv) \SuchThat{$\LPrv \in \LPrvS$} \label{alg:secm:getAttestationReport}}{
        \Return {attestation\_report}
    }
\end{comment}

\BlankLine
% 
% \UponEv(\tcp*[f]{The CONFINE protocol begins -- \textit{initialization} phase in \cref{fig:init})}){$\langle \SecM.\Compo{LogRequester}, \Mesg{Init} \:|\: \LPrvS, \SegSize \rangle$}{
% 	\ForEach(\tcp*[f]{For every \Compo{Provisioner} $\LPrv$}){$\LPrv \in \LPrvS$}{%
% 		\Trigger{$\langle \LPrv.\Compo{LogProvider}, \Mesg{CaseRefsReq} \:|\: \SecM \rangle$\label{alg:secm:CaseRefsReq:call}} \tcp*{Request \LPrv's case references (see \crefalgln[alg:lprv]{alg:lprv:CasesRefReq})}
% 	}
% 	\Upon(\tcp*[f]{Once all \Compo{Provisioner}s have answered with their case references}){$|\LPrvS| = |\textrm{dom}(\LPrvMap)|$}{%
% 		\lForEach%(\tcp*[f]{For every reference to the \Compo{Log Provider} $\LPrv'$})
% 		{$\LPrv \in \LPrvS$}{
% 			\Trigger{$\langle \LPrv.\Compo{LogProvider}, \Mesg{CasesReq} \:|\: \SecM, \SegSize, \LPrvMap[\LPrv] \rangle$\label{alg:secm:CasesReq:call}}
% 			\tcp*[f]{Request their cases (see \crefalgln[alg:lprv]{alg:lprv:CasesReq})}
% 			%\tcc*{Request the cases that are provided by $\LPrv'$. Before sending them, $\LPrv'$ will trigger \Mesg{AttestReportReq} in return, to attest the \Compo{Secure Miner}.}
% 		}
% 	}
% }
% \UponEv(\tcp*[f]{{\SecM} receives the case references from {\LPrv} (see \crefalgln[alg:lprv]{alg:lprv:sendRefs})}){$\langle \SecM.\Compo{LogRequester}, \Mesg{CaseRefsRes} \:|\: \LPrv, \CIdS \rangle$ \SuchThat{$\LPrv \in \LPrvS$} \label{alg:secm:CaseRefsRes}}{
% 	\ForEach(\tcp*[f]{For every case reference $\CId$} received in {\CIdS}){$\CId \in \CIdS$}{%
% 		$\CIDMap[\CId] \gets \CIDMap[\CId] \cup \{\LPrv\} $ \tcp*{Add $\LPrv$ to the set of provisioners for case $\CId$ in $\CIDMap$}
% 	}
% 	$\LPrvMap[\LPrv] \gets \LPrvMap[\LPrv] \cup \CIdS $ \tcp*{Register the references of the cases provided by $\LPrv$ in $\LPrvMap$}
% }

% \UponEv(\tcp*[f]{$\SecM$ gets a segment from {\LPrv} (\crefalgln[alg:lprv]{alg:lprv:sendSegs}) -- \textit{data transmission} in \cref{fig:transmission})}){$\langle \SecM.\Compo{LogReceiver}, \Mesg{CasesRes} \:|\: \LPrv, \Segm \rangle$ \SuchThat{$\LPrv \in \LPrvS$} \label{alg:secm:CasesRes} }{
% 	% See {\LaTeX} comments\\
% 	% Per ogni pezzo-di-caso ricevuto nel segmento, controlla che il provider sia stato dichiarato in possesso di esso
% 	% SE PMap ha ancora il CID
% 	% Aggiungi il pezzo-di-caso alla lista di pezzi-di-caso associati a quell'id
% 	% Togli il CID del pezzo-di-caso da PMap in P
% 	% Togli il P dal CIDMap
% 	% upon CIDMap vuoto in un CID, mergia e yielda il caso
% 	\ForEach(\tcp*[f]{For every $\CasP_\CId$ in the delivered segment $\Segm$, each associated with a \CId}){$\CasP_\CId \in \Segm$}{%
% 		\If(\tcp*[f]{If {\LPrv} has declared the ownership of {\CId} (see \crefalgln{alg:secm:CaseRefsRes})}){$\CId \in \LPrvMap[\LPrv]$}  {%
% 			$\LPrvMap[\LPrv] \gets \LPrvMap[\LPrv] \,\setminus\, \{\CId\}$  \tcp*[r]{\raggedright Remove {\CId} from the set of case references to be provided by {\LPrv}}
% 			$\CIDMap[\CId] \gets \CIDMap[\CId] \,\setminus\, \{\LPrv\}$ \tcp*[r]{Remove $\LPrv$ from the set of $\CId$ provisioners}
% 			$\Compo{LogManager}.\Call{mergeAndStore}\left(\CStor, \CasP_\CId\right)$ \tcp*[r]{Update the case via $\Merge$ and store the result in {\CStor}}
% 		}
% 	}
% }

% \Upon(\tcp*[f]{When all the pieces of some $\CId$ have arrived} to \SecM){$\CIDMap[\CId]= \emptyset$ for some $\CId \in \textrm{dom}(\CIDMap)$} {%
% 	$\textrm{dom}(\CIDMap) \gets \textrm{dom}(\CIDMap) \,\setminus\, \{\CId\}$\tcp*[r]{Remove $\CId$ from the domain of cases which still needs to be processed}
% 	\Yield{\CStor[\CId] \To{}} \SecM.\Compo{LogProcessor} \tcp*[f]{Forward the $\CId$ to the \Compo{Log Processor} for mining -- \textit{computation} phase in \cref{fig:computation}}
% }
\UponEv(\tcp*[f]{The \Compo{Log Requester} of {\SecM} starts the CONFINE protocol -- \textit{initialization} phase in \cref{fig:init})}){$\langle \SecM, \Mesg{Init} \: |\: \LPrvS, \SegSize \rangle$ \label{alg:secm:init}}{
	\ForEach(\tcp*[f]{For every \Compo{Provisioner} $\LPrv$}){$\LPrv \in \LPrvS$}{%
		\Trigger{$\langle \AuthPtP, \Mesg{Send} \gg \LPrv\ \:|\: \Mesg{CasesRefReq} \rangle$\label{alg:secm:CaseRefsReq:call}} \tcp*{Request \LPrv's case references (see \crefalgln[alg:lprv]{alg:lprv:CasesRefReq})}
	}
	\Upon(\tcp*[f]{Once all \Compo{Provisioner}s have answered with their case references}){$|\LPrvS| = |\textrm{dom}(\LPrvMap)|$\label{alg:secm:respcollection}}{%
		\lForEach%(\tcp*[f]{For every reference to the \Compo{Log Provider} $\LPrv'$})
		{$\LPrv \in \LPrvS$}{
			\Trigger{$\langle \AuthPtP, \Mesg{Send} \gg {\LPrv}\:|\:\Mesg{CasesReq},\SegSize, \LPrvMap[\LPrv]\rangle$\label{alg:secm:CasesReq:call}}
			\tcp*[f]{Request their cases via {\AuthPtP} (see \crefalgln[alg:lprv]{alg:lprv:CasesReq})}
			%\tcc*{Request the cases that are provided by $\LPrv'$. Before sending them, $\LPrv'$ will trigger \Mesg{AttestReportReq} in return, to attest the \Compo{Secure Miner}.}
		}
	}
}

\UponEv(\tcp*[f]{{\SecM}'s \Compo{Log Requester} gets {\LPrv}'s case references via {\AuthPtP} (\crefalgln[alg:lprv]{alg:lprv:sendRefs})}){$\langle \AuthPtP, \Mesg{Deliver} \ll \LPrv \:|\: \Mesg{CasesRefRes}, \CIdS\rangle$ \SuchThat{$\LPrv \in \LPrvS$} \label{alg:secm:CaseRefsRes}}{
	\ForEach(\tcp*[f]{For every case reference $\CId$} received in {\CIdS}){$\CId \in \CIdS$}{%
		$\CIDMap[\CId] \gets \CIDMap[\CId] \cup \{\LPrv\} $ \tcp*{Add $\LPrv$ to the set of provisioners for case $\CId$ in $\CIDMap$}
	}
	$\LPrvMap[\LPrv] \gets \LPrvMap[\LPrv] \cup \CIdS $ \tcp*{Register the references of the cases provided by $\LPrv$ in $\LPrvMap$}
}

\UponEv(\tcp*[f]{$\SecM$'s \Compo{Log Receiver} gets a segment from {\LPrv} via {\AuthPtP} (\crefalgln[alg:lprv]{alg:lprv:sendSegs}))}){$\langle \AuthPtP, \Mesg{Deliver} \:|\: \LPrv, [\Mesg{CasesRes},\Segm] \rangle$ \SuchThat{$\LPrv \in \LPrvS$} \label{alg:secm:CasesRes} }{
	\ForEach(\tcp*[f]{For every $\CasP_\CId$ in the delivered segment $\Segm$, each associated with a \CId -- \textit{data transmission} phase in \cref{fig:transmission}}){$\CasP_\CId \in \Segm$}{%
		\If(\tcp*[f]{If {\LPrv} has declared the ownership of {\CId} (see \crefalgln{alg:secm:CaseRefsRes})}){$\CId \in \LPrvMap[\LPrv]$}  {%
			$\LPrvMap[\LPrv] \gets \LPrvMap[\LPrv] \,\setminus\, \{\CId\}$  \tcp*[r]{\raggedright Remove {\CId} from the set of case references to be provided by {\LPrv}}
			$\CIDMap[\CId] \gets \CIDMap[\CId] \,\setminus\, \{\LPrv\}$ \tcp*[r]{Remove $\LPrv$ from the set of $\CId$ provisioners}
			$\SecM.\Compo{LogManager}.\Call{mergeAndStore}\left(\CStor, \CasP_\CId\right)$ \tcp*[r]{Update the case via $\Merge$ and store the result in {\CStor}\label{alg:secm:mergeAndStore}}
		}
	}
}

\Upon(\tcp*[f]{When all the pieces of some $\CId$ have arrived} to \SecM's \Compo{Log Manager}){$\CIDMap[\CId]= \emptyset$ for some $\CId \in \textrm{dom}(\CIDMap)$\label{alg:secm:computation}} {%
	$\textrm{dom}(\CIDMap) \gets \textrm{dom}(\CIDMap) \,\setminus\, \{\CId\}$\tcp*[r]{Remove $\CId$ from the domain of cases which still needs to be processed}
	\Yield{\CStor[\CId] \To{}} \SecM.\Compo{LogProcessor} \tcp*[f]{Forward the case $\CId$ to the \Compo{Log Processor} of {\SecM} for mining -- \textit{computation} phase in \cref{fig:computation}\label{alg:secm:yield}}
}

==> content/tables/coefficentsTestTable.tex <==
\begin{subfigure}{0.49\textwidth}
\label{tab:metrics}
  \centering
   \subfloat[Scalability metrics]{%
   \resizebox{0.94\textwidth}{!}{%
    \begin{tabular}{l c c c c}
       \toprule
         & \textbf{Linear Corr}.  & \textbf{Linear Slope}  & \textbf{R$^2$} & \textbf{Speedup}\\
         \midrule
         \multicolumn{5}{c}{\textbf{Number of cases test}} \\
         \midrule
         Seg. size 100& 0.9948&0.0013&0.6822&0.1890 \\
         Seg. size 1000&0.9812&0.0010&0.8682&0.2928\\
         Seg. size 10000&0.8791&0.0068&0.9303&0.0675\\
         \midrule
         \multicolumn{5}{c}{\textbf{Max events test}} \\
         \midrule
         Seg. size 100&0.9923& 0.0980&0.8291&0.0929\\
         Seg. size 1000&0.9769&0.0821&0.9043&0.2425\\
         Seg. size 10000&0.8577&0.1518&0.9386&0.3258\\
         \midrule
         \multicolumn{5}{c}{\textbf{Number of provisioner organizations test}} \\
         \midrule
         Seg. size 100&0.9884&0.3184&0.8577&0.5103\\
         Seg. size 1000&0.9799&0.5174&0.7902&0.5211\\
         Seg. size 10000&0.9521&0.6102&0.6977&0.6101\\
         \bottomrule
    \end{tabular}
    }
  } 


==> content/threatmodel.tex <==
\subsection{Threat Model}
\label{sec:thretmodel}
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{content//figures/threatmodel.pdf}
    \caption{Data flow diagram employed for our threat model}
    \label{fig:threatmodel:dataflow}
\end{figure}
\begin{table}[t]
\resizebox{\textwidth}{!}{%
    \centering
    \begin{tabular}{llll}\toprule
        \textbf{ID} & \textbf{Trust boundary}& \textbf{Type}  & \textbf{Threat description}\\ \midrule
        T01& \multirow{3}{*}{\makecell[l]{TBB01}}& Information disclosure  & The attacker accesses the \Compo{Secure Miner}'s memory location to leak the event logs\\ %01
        T02& & Tampering  & The attacker meddles the source code of the \Compo{Secure Miner} or its event log data\\ %02
        T03& & Elevation of privileges  & The attacker gains the rights to run in the same environment of the \Compo{Secure Miner}\\\midrule %03
       % T04& & Denial of service  & The \Compo{Secure Miner} crashes, halts or stops\\ \midrule %04
        T04& \multirow{3}{*}{\makecell[l]{TBA01}}& Spoofing  & The attacker impersonates a \Compo{Secure Miner} to gain access to the \Compo{Provisioner}'s log\\ %05
        T05& & Spoofing  & The attacker impersonates a \Compo{Provisioner} to communicate with the \Compo{Secure Miner}\\ %06
        %T07& & Denial of service &The \Compo{Secure Miner} floods the \Compo{Provisioner} with log requests\\ %07
        T06& & Information disclosure & The attacker sniffs the data exchanged between the \Compo{Provisioner} and the \Compo{Secure Miner}\\\midrule %08
       % T09& & Tampering & The attacker alters the data flow between the \Compo{Provisioner} and the \Compo{Secure Miner}\\ \midrule %09
        T07& \multirow{3}{*}{\makecell[l]{TBA02}}& Spoofing   & The attacker impersonates a legitimate interactor to use the \Compo{Secure Miner}\\ %10
        T08&     & Tampering  & The intra-organizational interactor sends malicious input to the \Compo{Secure Miner}\\ %11
        T09&     & Information disclosure  & The attacker sniffs messages between the \Compo{Secure Miner} and the intra-organizational party  \\ %11
       % T09&     & Information disclosure  & The attacker sniffs the messages between the interactor and the \Compo{Secure Miner}\\ %12
        \bottomrule
    \end{tabular}
    \caption{Main vulnerabilities in the CONFINE architecture}
    \label{table:threatmodel:threats}
}
\end{table}
This section is dedicated to identifying potential threats that could compromise data secrecy within our high-level architecture. The threats outlined in this section establish the security requirements that the CONFINE deployment must meet in the subsequent section (\cref{sec:deployment}).
%In the following section, we identify the threats that can jeopardize the proper functioning of the CONFINE architecture. 

Our threat analysis is based upon the theoretical foundation of the \textit{STRIDE} framework \cite{DBLP:journals/re/ScandariatoWJ15}. This conceptual model groups the threats into six categories: \textit{spoofing} (i.e., the impersonation of a legitimate entity), tampering (i.e., the modification of data to alter its integrity), \textit{repudiation} (i.e., the denial of performing a particular action), \textit{information disclosure} (i.e., the exposure of sensitive data), \textit{denial of service} (i.e., the disruption or degradation of availability) and \textit{elevation of privileges} (i.e., the misappropriation of a higher level of rights).

With the help of the dataflow diagram (DFD) depicted in \cref{fig:threatmodel:dataflow}, we demarcate the \textit{trust boundaries} among the CONFINE components. In our DFD, a trust boundary box (the orange dotted square) groups entities with mutual trust. Differently, trust boundary arches (red dashed lines) mark the transitions of trust level on the occasion of data exchanges (the black arrows) between untrusted parties. The opening side of each arch denotes the parties holding trust in the data exchange interaction. We identify four trust boundaries: the \Compo{Secure Miner}'s trust boundary box (\textbf{TBB01}), the inter-organizational trust boundary arch (\textbf{TBA01}), the intra-organizational trust boundary arch (\textbf{TBA02}), and the \Compo{Provisioner}'s trust boundary box. As a result of our analysis, we collect in \cref{table:threatmodel:threats} the threats in CONFINE according to the STRIDE taxonomy.

In our examination, we exclude the security considerations pertaining to \Compo{Provisioner}'s trust boundary boxes (the gray dotted square in \cref{fig:threatmodel:dataflow}), as menaces targeting event logs in their native organizational domain fall beyond the scope of this study. Hence, we concentrate our endeavors on preserving data secrecy when log partitions (introduced in \cref{def:partition}) cross their organizational confines. 

We address the identified threats, grouping them according to the trust boundary they refer to.

The trust boundary box TBB01 encloses the components of the \Compo{Secure Miner}. The spectrum of potential attacks targeting this trust domain aims to undermine the isolation layer that separates the components of the \Compo{Secure Miner}, including provisioners' log partitions, from untrusted entities. %Attacks against this trust boundary may emanate from a generic entity, which could be either intra-organizational (i.e., within the same organization as the \Compo{Secure Miner}) or inter-organizational (i.e., beyond the boundaries of the \Compo{Secure Miner}'s organization). 
To expose confidential information, a malicious actor might gain access to the memory allocated to the \Compo{Secure Miner}, for instance, through a \textit{direct memory access} attack \cite{DBLP:conf/cms/EckertPK13}, thereby revealing event logs' sensitive information (\textbf{T01}). Tampering threats materialize in the form of manipulating the \Compo{Secure Miner}'s source code and event log data to induce misbehaviors or introduce vulnerabilities (\textbf{T02}). Furthermore, a malicious actor could obtain the necessary privileges, such as through \textit{kernel exploits} \cite{DBLP:conf/securecomm/XiaoHW15a}, to execute code within the isolated context of the \Compo{Secure Miner}, potentially resulting in unauthorized access or the injection of malicious code (\textbf{T03}). %A denial of service attack may be employed by a malicious entity to crash, halt, or disrupt the functioning of the \Compo{Secure Miner}, thereby hindering the aggregation event log data correctly and the outsourcing of result analytics (\textbf{T04}). 

TBA01 encompasses inter-organizational concerns regarding the data exchange between the \Compo{Secure Miner} and the \Compo{Provisioner}s. In our DFD, this arch is open towards the \Compo{Provisioner}, thus indicating that this component is the trusted party in the information trade. %In this regard, an attacker may generate threats aimed at disrupting the data transmission process responsible for delivering \Compo{Provisioner}s' log partitions to the \Compo{Secure Miner}. 
A spoofing attack could result in the \Compo{Secure Miner} being impersonated, leading to the improper reception of the \Compo{Provisioner}'s log partition (\textbf{T04}). Similarly, if an attacker successfully impersonates a \Compo{Provisioner}, it could send fictitious event logs to manipulate the data analytics output (\textbf{T05}). %Furthermore, the log delivery service may be interrupted by one or more malicious entities generating an excessive number of data requests (e.g., through \textit{DDoS} \cite{DBLP:journals/ijdsn/MahjabinXSJ17} and \textit{TCP-SYN floodding} \cite{DBLP:journals/wpc/SwamiDR21} attacks) targeting the \Compo{Provisioner} (\textbf{T07}). 
A man-in-the-middle attack, such as eavesdropping and packet sniffing \cite{DBLP:journals/jocs/LiXDZCW15}, could allow a third-party actor to monitor the data flow between the \Compo{Secure Miner} and the \Compo{Provisioner}, thereby enabling the disclosure confidential information (\textbf{T06}).%or the alteration of meaningful data (\textbf{T09}).

The TBA02 trust boundary arch involves the interaction between the \Compo{Secure Miner} and a generic intra-organizational interactor (e.g., a user or a process within the same organization of the miner). As shown in our diagram, the intra-organizational actor is the untrusted party of this interaction. A spoofing threat holds the potential for an assailant to emulate a legitimate interactor, enabling them to engage with the \Compo{Secure Miner} (\textbf{T07}). Furthermore, there exists a risk wherein a legitimate interactor, motivated by malicious intent, may introduce deleterious inputs to the \Compo{Secure Miner}, including the submission of corrupted data or issuance of dangerous commands (\textbf{T08}). The emergence of information disclosure threats transpires when a malicious actor intercepts messages exchanged between a legitimate interactor and the \Compo{Secure Miner}, thereby attaining unauthorized access to sensitive information, including credentials or reserved outputs (\textbf{T09}).

In the subsequent \cref{sec:deployment}, we leverage the newly identified threats to instantiate the high-level architecture and devise an interaction protocol that fulfills the discussed security requirements. Therefore, in \cref{sec:discussion:security}, we assess the security of the CONFINE deployment by showcasing how our instantiation addresses each of these threats.


